The JADES Transient Survey: Discovery and Classification of Supernovae in the JADES Deep Field

The JWST Advanced Deep Extragalactic Survey (JADES) is a multi-cycle JWST program that has taken among the deepest near-/mid-infrared images to date (down to $\sim$30 ABmag) over $\sim$25 arcmin$^2$ in the GOODS-S field in two sets of observations with one year of separation. This presented the first opportunity to systematically search for transients, mostly supernovae (SNe), out to $z$$>$2. We found 79 SNe: 38 at $z$$<$2, 23 at 2$<$$z$$<$3, 8 at 3$<$$z$$<$4, 7 at 4$<$$z$$<$5, and 3 with undetermined redshifts, where the redshifts are predominantly based on spectroscopic or highly reliable JADES photometric redshifts of the host galaxies. At this depth, the detection rate is $\sim$1-2 per arcmin$^2$ per year, demonstrating the power of JWST as a supernova discovery machine. We also conducted multi-band follow-up NIRCam observations of a subset of the SNe to better constrain their light curves and classify their types. Here, we present the survey, sample, search parameters, spectral energy distributions (SEDs), light curves, and classifications. Even at $z$$\geq$2, the NIRCam data quality is high enough to allow SN classification via multi-epoch light-curve fitting with confidence. The multi-epoch SN sample includes a Type Ia SN at $z_{\mathrm{spec}}$$=$2.90, Type IIP SN at $z_{\mathrm{spec}}$$=$3.61, and a Type Ic-BL SN at $z_{\mathrm{spec}}$$=$2.83. We also found that two $z$$\sim$16 galaxy candidates from the first imaging epoch were actually transients that faded in the second epoch, illustrating the possibility that moderate/high-redshift SNe could mimic high-redshift dropout galaxies.

==> tab/tab_JD22_aperture_phot.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{cccccccccc}
\tablecaption{JD22 Epoch1-Epoch2 SN photometry}
\tablehead{
\colhead{ID} & \colhead{F090W} & \colhead{F115W} & \colhead{F150W} & \colhead{F200W} & \colhead{F277W} & \colhead{F335M} & \colhead{F356W} & \colhead{F410M} & \colhead{F444W} \\
\colhead{} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)}
} 
\startdata
JD22.1  & $>$30.2        & $>$30.6        & $>$30.5        & $>$30.6        & 30.18$\pm$0.16 & 29.88$\pm$0.21 & 29.96$\pm$0.13 & $>$30.1        & 30.17$\pm$0.20 \\
JD22.2  & $>$30.2        & $>$30.6        & $>$30.5        & $>$30.6        & 29.69$\pm$0.09 & $>$30.1        & 29.50$\pm$0.08 & $>$30.1        & 30.16$\pm$0.16 \\
JD22.3  & $>$30.2        & $>$30.6        & 29.32$\pm$0.22 & \nodata        & 28.44$\pm$0.05 & \nodata        & \nodata        & 28.67$\pm$0.15 & 29.39$\pm$0.19 \\
JD22.4  & $>$30.2        & $>$30.6        & $>$30.5        & 28.95$\pm$0.07 & 27.78$\pm$0.02 & 27.54$\pm$0.03 & 27.65$\pm$0.03 & 27.75$\pm$0.05 & 27.70$\pm$0.04 \\
JD22.5  & $>$30.2        & $>$30.6        & $>$30.5        & $>$30.6        & 30.09$\pm$0.12 & $>$30.1        & 30.43$\pm$0.27 & $>$30.1        & $>$30.3        \\
JD22.6  & $>$30.2        & $>$30.6        & $>$30.5        & 29.69$\pm$0.27 & 29.26$\pm$0.17 & 29.44$\pm$0.31 & 29.53$\pm$0.29 & $>$30.1        & 29.37$\pm$0.24 \\
JD22.7  & 29.47$\pm$0.22 & 29.17$\pm$0.11 & 29.25$\pm$0.16 & 29.43$\pm$0.15 & $>$30.7        & 30.06$\pm$0.32 & $>$30.6        & $>$30.1        & $>$30.3        \\
JD22.8  & $>$30.2        & $>$30.6        & $>$30.5        & 30.51$\pm$0.32 & 30.29$\pm$0.14 & $>$30.1        & $>$30.6        & $>$30.1        & $>$30.3        \\
JD22.9  & $>$30.2        & $>$30.6        & $>$30.5        & 28.82$\pm$0.10 & 28.46$\pm$0.06 & 27.96$\pm$0.07 & 28.15$\pm$0.07 & 28.18$\pm$0.08 & 28.24$\pm$0.08 \\
JD22.10 & $>$30.2        & 30.22$\pm$0.32 & 30.12$\pm$0.36 & 28.70$\pm$0.11 & 28.35$\pm$0.06 & 28.88$\pm$0.19 & 28.62$\pm$0.14 & 28.75$\pm$0.25 & 28.90$\pm$0.15 \\
JD22.11 & $>$30.2        & 30.22$\pm$0.28 & $>$30.5        & 30.36$\pm$0.38 & 29.77$\pm$0.16 & 29.50$\pm$0.17 & 29.32$\pm$0.12 & 29.25$\pm$0.15 & 30.13$\pm$0.30 \\
JD22.12 & $>$30.2        & $>$30.6        & $>$30.5        & $>$30.6        & 29.78$\pm$0.11 & 29.24$\pm$0.12 & 29.17$\pm$0.08 & 29.04$\pm$0.10 & 29.53$\pm$0.17 \\
JD22.13 & $>$30.2        & $>$30.6        & $>$30.5        & 29.76$\pm$0.26 & 29.41$\pm$0.15 & 29.11$\pm$0.19 & 28.96$\pm$0.11 & 28.66$\pm$0.14 & 28.91$\pm$0.12 \\
JD22.14 & $>$30.2        & $>$30.6        & $>$30.5        & $>$30.6        & 29.82$\pm$0.09 & 29.82$\pm$0.17 & 30.02$\pm$0.14 & 30.07$\pm$0.24 & 29.87$\pm$0.15 \\
JD22.15 & $>$30.2        & $>$30.6        & 28.59$\pm$0.06 & 28.15$\pm$0.05 & 28.28$\pm$0.06 & 28.76$\pm$0.17 & 28.61$\pm$0.15 & 28.86$\pm$0.20 & 28.97$\pm$0.16 \\
JD22.16 & $>$30.2        & 30.52$\pm$0.45 & 29.60$\pm$0.25 & 29.86$\pm$0.33 & 29.18$\pm$0.08 & 29.23$\pm$0.13 & 29.18$\pm$0.09 & 29.63$\pm$0.24 & 29.69$\pm$0.18 \\
JD22.17 & $>$30.2        & $>$30.6        & 28.69$\pm$0.06 & 28.04$\pm$0.04 & 28.11$\pm$0.02 & 28.19$\pm$0.04 & 28.20$\pm$0.03 & 28.26$\pm$0.05 & 28.46$\pm$0.06 \\
JD22.18 & $>$30.2        & 29.89$\pm$0.18 & 28.78$\pm$0.06 & 27.78$\pm$0.04 & 27.17$\pm$0.03 & 27.11$\pm$0.04 & 27.00$\pm$0.04 & 27.01$\pm$0.06 & 27.14$\pm$0.08 \\
JD22.19 & 29.83$\pm$0.20 & 28.93$\pm$0.07 & 28.31$\pm$0.04 & 27.90$\pm$0.03 & 27.73$\pm$0.02 & 27.72$\pm$0.02 & 27.73$\pm$0.03 & 28.00$\pm$0.06 & 27.91$\pm$0.05 \\
JD22.20 & $>$30.2        & $>$30.6        & 30.17$\pm$0.34 & 29.93$\pm$0.28 & 29.59$\pm$0.11 & $>$30.1        & 29.59$\pm$0.12 & 29.50$\pm$0.26 & 30.23$\pm$0.39 \\
JD22.21 & 27.90$\pm$0.06 & 26.79$\pm$0.02 & 26.61$\pm$0.02 & 26.60$\pm$0.02 & 26.68$\pm$0.02 & 26.84$\pm$0.03 & 26.87$\pm$0.02 & 27.09$\pm$0.04 & 27.09$\pm$0.04 \\
JD22.22 & $>$30.2        & 30.31$\pm$0.25 & 30.08$\pm$0.20 & 29.79$\pm$0.18 & 29.93$\pm$0.14 & $>$30.1        & $>$30.6        & $>$30.1        & $>$30.3        \\
JD22.23 & 26.17$\pm$0.02 & 25.58$\pm$0.01 & 25.21$\pm$0.01 & 25.18$\pm$0.02 & 25.33$\pm$0.01 & 25.53$\pm$0.01 & 25.55$\pm$0.01 & 25.77$\pm$0.04 & 25.85$\pm$0.03 \\
JD22.24 & 26.96$\pm$0.02 & 26.29$\pm$0.01 & 26.42$\pm$0.01 & 26.74$\pm$0.03 & 27.21$\pm$0.01 & 27.59$\pm$0.04 & 27.72$\pm$0.02 & 27.95$\pm$0.05 & 28.09$\pm$0.05 \\
JD22.25 & 30.03$\pm$0.38 & 29.19$\pm$0.12 & 28.27$\pm$0.07 & 28.07$\pm$0.05 & 28.11$\pm$0.03 & 29.19$\pm$0.14 & 28.77$\pm$0.06 & 28.66$\pm$0.12 & 28.61$\pm$0.09 \\
JD22.26 & 29.78$\pm$0.20 & 29.65$\pm$0.17 & 28.93$\pm$0.10 & 28.88$\pm$0.07 & 29.10$\pm$0.09 & 29.02$\pm$0.11 & 29.23$\pm$0.10 & 29.28$\pm$0.14 & 29.30$\pm$0.13 \\
JD22.27 & 28.12$\pm$0.07 & 27.93$\pm$0.04 & 27.88$\pm$0.05 & 27.86$\pm$0.07 & 28.22$\pm$0.13 & 28.65$\pm$0.28 & 28.76$\pm$0.33 & 28.91$\pm$0.42 & 28.89$\pm$0.48 \\
JD22.28 & $>$30.2        & $>$30.6        & $>$30.5        & 29.95$\pm$0.21 & 30.30$\pm$0.14 & $>$30.1        & 30.47$\pm$0.21 & $>$30.1        & 30.17$\pm$0.26 \\
JD22.29 & 30.05$\pm$0.38 & 30.37$\pm$0.32 & 29.07$\pm$0.13 & 29.79$\pm$0.22 & 29.44$\pm$0.10 & $>$30.1        & 29.95$\pm$0.22 & 29.84$\pm$0.31 & 29.89$\pm$0.25 \\
JD22.30 & $>$30.2        & $>$30.6        & 29.82$\pm$0.25 & 29.89$\pm$0.23 & 30.09$\pm$0.17 & $>$30.1        & 29.89$\pm$0.19 & 29.43$\pm$0.16 & 29.81$\pm$0.19 \\
JD22.31 & 28.70$\pm$0.10 & 28.16$\pm$0.06 & 27.86$\pm$0.05 & 28.31$\pm$0.09 & 27.91$\pm$0.12 & 29.01$\pm$0.36 & 28.37$\pm$0.20 & 27.59$\pm$0.17 & 27.83$\pm$0.24 \\
JD22.32 & $>$30.2        & $>$30.6        & $>$30.5        & 30.51$\pm$0.42 & 29.46$\pm$0.09 & 29.38$\pm$0.15 & 29.25$\pm$0.10 & 29.16$\pm$0.15 & 29.49$\pm$0.17 \\
JD22.33 & 29.10$\pm$0.13 & 28.64$\pm$0.06 & 28.95$\pm$0.11 & 29.06$\pm$0.11 & 29.84$\pm$0.11 & $>$30.1        & $>$30.6        & $>$30.1        & $>$30.3        \\
JD22.34 & 29.87$\pm$0.35 & 28.13$\pm$0.07 & 27.71$\pm$0.05 & 27.63$\pm$0.05 & 27.43$\pm$0.04 & 27.77$\pm$0.07 & 27.73$\pm$0.07 & 27.83$\pm$0.09 & 28.06$\pm$0.08 \\
JD22.35 & $>$30.2        & $>$30.6        & $>$30.5        & 30.14$\pm$0.27 & 29.62$\pm$0.07 & 29.43$\pm$0.10 & 30.15$\pm$0.15 & $>$30.1        & 29.90$\pm$0.14 \\
JD22.36 & $>$30.2        & 30.10$\pm$0.18 & 28.62$\pm$0.06 & 28.00$\pm$0.04 & 27.85$\pm$0.02 & 27.98$\pm$0.04 & 27.96$\pm$0.03 & 28.11$\pm$0.05 & 28.14$\pm$0.06 \\
JD22.37 & 27.09$\pm$0.04 & 26.35$\pm$0.02 & 26.09$\pm$0.02 & 26.24$\pm$0.03 & 26.60$\pm$0.04 & 26.75$\pm$0.07 & 26.88$\pm$0.06 & 26.95$\pm$0.08 & 27.29$\pm$0.08 \\
JD22.38 & $>$30.2        & $>$30.6        & $>$30.5        & 30.16$\pm$0.34 & 29.06$\pm$0.11 & 29.76$\pm$0.31 & 29.18$\pm$0.10 & 29.18$\pm$0.17 & 29.56$\pm$0.24 \\
JD22.39 & $>$30.2        & $>$30.6        & 30.07$\pm$0.50 & 28.00$\pm$0.09 & 27.22$\pm$0.05 & 27.03$\pm$0.06 & 26.90$\pm$0.06 & 27.16$\pm$0.08 & 27.21$\pm$0.07 \\
JD22.40 & $>$30.2        & $>$30.6        & 30.30$\pm$0.28 & 29.91$\pm$0.23 & 29.78$\pm$0.12 & $>$30.1        & 29.74$\pm$0.13 & $>$30.1        & 29.72$\pm$0.17 \\
JD22.41 & 29.41$\pm$0.30 & 28.36$\pm$0.08 & 28.44$\pm$0.11 & 28.24$\pm$0.10 & 28.64$\pm$0.25 & 28.29$\pm$0.18 & 28.08$\pm$0.13 & 27.32$\pm$0.06 & 27.49$\pm$0.07 \\
JD22.42 & 27.27$\pm$0.03 & 26.68$\pm$0.01 & 26.46$\pm$0.02 & 26.49$\pm$0.02 & 26.83$\pm$0.07 & 27.09$\pm$0.05 & 27.10$\pm$0.05 & 27.37$\pm$0.08 & 27.42$\pm$0.09 \\
JD22.43 & 29.49$\pm$0.19 & 29.13$\pm$0.08 & 29.12$\pm$0.09 & 29.54$\pm$0.15 & 29.82$\pm$0.11 & $>$30.1        & 30.55$\pm$0.25 & $>$30.1        & $>$30.3        \\
JD22.44 & $>$30.2        & 29.40$\pm$0.11 & 28.53$\pm$0.05 & 28.28$\pm$0.05 & 28.80$\pm$0.05 & \nodata        & \nodata        & 28.75$\pm$0.11 & 28.82$\pm$0.09 \\
JD22.45 & 29.28$\pm$0.21 & 29.17$\pm$0.12 & 29.24$\pm$0.20 & 29.80$\pm$0.23 & 29.83$\pm$0.14 & 29.79$\pm$0.28 & 29.71$\pm$0.15 & 29.49$\pm$0.25 & $>$30.3        \\ 
\sidehead{Excluded from sample} 
JD22.46 & $>$30.2        & 30.26$\pm$0.72 & 28.91$\pm$0.12 & \nodata        & 27.95$\pm$0.04 & 28.72$\pm$0.10 & 28.95$\pm$0.12 & 29.01$\pm$0.15 & 28.87$\pm$0.15 
\enddata

\label{tab_JD22_photometry}

\end{deluxetable*}
\end{longrotatetable}

==> tab/tab_JD23_aperture_phot.tex <==
\begin{longrotatetable}
\begin{deluxetable}{cccccccccc}
\tablecaption{JD23 Epoch2-Epoch1 SN photometry}
\tablehead{
\colhead{ID} & \colhead{F090W} & \colhead{F115W} & \colhead{F150W} & \colhead{F200W} & \colhead{F277W} & \colhead{F335M} & \colhead{F356W} & \colhead{F410M} & \colhead{F444W} \\
\colhead{} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)}
} 
\startdata
JD23.1  & $>$30.2        & $>$30.6        & $>$30.5        & $>$30.6        & 29.17$\pm$0.11 & 28.98$\pm$0.14 & 28.65$\pm$0.07 & 28.69$\pm$0.11 & 28.48$\pm$0.08 \\
JD23.2  & $>$30.2        & $>$30.6        & $>$30.5        & $>$30.6        & 29.75$\pm$0.14 & 29.32$\pm$0.14 & 29.30$\pm$0.10 & 29.70$\pm$0.25 & 29.97$\pm$0.26 \\
JD23.3  & 29.73$\pm$0.24 & 29.10$\pm$0.10 & 28.63$\pm$0.08 & 28.63$\pm$0.08 & 28.73$\pm$0.05 & 28.84$\pm$0.07 & 29.30$\pm$0.10 & 28.74$\pm$0.10 & 29.14$\pm$0.14 \\
JD23.4  & $>$30.2        & $>$30.6        & $>$30.5        & $>$30.6        & 29.30$\pm$0.07 & 29.23$\pm$0.12 & 29.30$\pm$0.11 & 29.55$\pm$0.19 & 29.33$\pm$0.14 \\
JD23.5  & $>$30.2        & $>$30.6        & $>$30.5        & $>$30.6        & 29.62$\pm$0.10 & 29.33$\pm$0.13 & 29.94$\pm$0.17 & 29.24$\pm$0.16 & 29.20$\pm$0.10 \\
JD23.6  & $>$30.2        & 29.66$\pm$0.19 & 28.67$\pm$0.08 & 28.03$\pm$0.05 & 27.92$\pm$0.03 & 28.03$\pm$0.05 & 27.98$\pm$0.03 & 28.23$\pm$0.07 & 28.25$\pm$0.07 \\
JD23.7  & $>$30.2        & 30.01$\pm$0.28 & $>$30.5        & 29.06$\pm$0.16 & 28.63$\pm$0.17 & 28.75$\pm$0.16 & 28.35$\pm$0.11 & 28.20$\pm$0.11 & 28.34$\pm$0.12 \\
JD23.8  & $>$30.2        & $>$30.6        & $>$30.5        & 30.04$\pm$0.27 & 29.38$\pm$0.09 & $>$30.1        & 29.58$\pm$0.11 & 29.36$\pm$0.14 & 30.17$\pm$0.22 \\
JD23.9  & $>$30.2        & 30.55$\pm$0.26 & 29.96$\pm$0.18 & 29.52$\pm$0.13 & 28.88$\pm$0.03 & 28.89$\pm$0.07 & 28.93$\pm$0.05 & 28.76$\pm$0.09 & 29.09$\pm$0.07 \\
JD23.10 & $>$30.2        & 29.29$\pm$0.16 & 29.00$\pm$0.14 & 28.59$\pm$0.09 & 29.04$\pm$0.07 & 28.75$\pm$0.10 & 28.79$\pm$0.08 & 29.40$\pm$0.20 & 29.12$\pm$0.14 \\
JD23.11 & $>$30.2        & $>$30.6        & 30.27$\pm$0.34 & 28.97$\pm$0.10 & 28.32$\pm$0.04 & 28.12$\pm$0.05 & 28.14$\pm$0.04 & 28.37$\pm$0.08 & 28.21$\pm$0.07 \\
JD23.12 & $>$30.2        & $>$30.6        & 29.69$\pm$0.16 & 29.68$\pm$0.17 & 29.70$\pm$0.08 & $>$30.1        & 29.90$\pm$0.15 & 29.96$\pm$0.20 & $>$30.3        \\
JD23.13 & $>$30.2        & 29.45$\pm$0.17 & 28.93$\pm$0.12 & 29.06$\pm$0.15 & 29.02$\pm$0.20 & 28.98$\pm$0.18 & 29.34$\pm$0.26 & 28.53$\pm$0.20 & 28.41$\pm$0.17 \\
JD23.14 & $>$30.2        & 29.52$\pm$0.15 & 28.20$\pm$0.07 & 28.01$\pm$0.06 & 27.94$\pm$0.06 & 28.11$\pm$0.08 & 28.22$\pm$0.07 & 28.21$\pm$0.09 & 28.28$\pm$0.10 \\
JD23.15 & $>$30.2        & $>$30.6        & $>$30.5        & 28.23$\pm$0.12 & 27.82$\pm$0.03 & 27.46$\pm$0.02 & 27.61$\pm$0.02 & 27.67$\pm$0.04 & 27.85$\pm$0.05 \\
JD23.16 & $>$30.2        & 30.34$\pm$0.29 & 29.12$\pm$0.13 & 28.68$\pm$0.08 & 29.22$\pm$0.09 & 28.73$\pm$0.10 & 29.27$\pm$0.11 & 29.26$\pm$0.13 & 29.50$\pm$0.21 \\
JD23.17 & $>$30.2        & 30.20$\pm$0.34 & 28.61$\pm$0.09 & 28.42$\pm$0.07 & 28.17$\pm$0.05 & 28.59$\pm$0.08 & 28.57$\pm$0.06 & 28.58$\pm$0.11 & 28.41$\pm$0.09 \\
JD23.18 & $>$30.2        & 29.15$\pm$0.14 & 28.73$\pm$0.11 & \nodata        & 29.16$\pm$0.06 & 29.17$\pm$0.09 & 29.37$\pm$0.08 & 29.70$\pm$0.19 & 29.55$\pm$0.15 \\
JD23.19 & $>$30.2        & 30.01$\pm$0.28 & 28.54$\pm$0.07 & 27.79$\pm$0.04 & 27.91$\pm$0.03 & 27.93$\pm$0.03 & 27.97$\pm$0.03 & 28.25$\pm$0.06 & 28.23$\pm$0.04 \\
JD23.20 & $>$30.2        & $>$30.6        & 30.28$\pm$0.41 & 29.58$\pm$0.22 & 29.37$\pm$0.14 & 28.84$\pm$0.12 & 29.02$\pm$0.11 & 29.33$\pm$0.23 & 29.41$\pm$0.17 \\
JD23.21 & $>$30.2        & $>$30.6        & 28.79$\pm$0.16 & 28.38$\pm$0.16 & 29.18$\pm$0.41 & $>$30.1        & 29.22$\pm$0.59 & $>$30.1        & $>$30.3        \\
JD23.22 & 29.41$\pm$0.19 & 28.52$\pm$0.06 & 27.74$\pm$0.03 & 27.37$\pm$0.03 & 27.34$\pm$0.02 & 27.45$\pm$0.03 & 27.48$\pm$0.02 & 27.52$\pm$0.04 & 27.70$\pm$0.05 \\
JD23.23 & $>$30.2        & $>$30.6        & 29.56$\pm$0.30 & 28.94$\pm$0.14 & 29.37$\pm$0.30 & 29.51$\pm$0.40 & 29.52$\pm$0.40 & $>$30.1        & 29.79$\pm$0.52 \\
JD23.24 & $>$30.2        & 29.21$\pm$0.13 & 27.65$\pm$0.04 & 27.07$\pm$0.04 & 27.00$\pm$0.10 & 28.21$\pm$0.63 & 28.02$\pm$0.61 & 28.90$\pm$1.02 & 27.92$\pm$0.47 \\
JD23.25 & $>$30.2        & $>$30.6        & $>$30.5        & 28.95$\pm$0.11 & 28.75$\pm$0.10 & 28.66$\pm$0.12 & 28.92$\pm$0.09 & 28.79$\pm$0.15 & 29.13$\pm$0.24 \\
JD23.26 & 26.97$\pm$0.02 & 26.97$\pm$0.02 & 27.06$\pm$0.02 & 27.23$\pm$0.03 & 27.65$\pm$0.05 & 28.02$\pm$0.10 & 27.98$\pm$0.08 & 28.22$\pm$0.14 & 28.26$\pm$0.12 \\
JD23.27 & $>$30.2        & $>$30.6        & $>$30.5        & 30.30$\pm$0.25 & 29.02$\pm$0.08 & 28.67$\pm$0.09 & 28.76$\pm$0.07 & 29.43$\pm$0.19 & 29.01$\pm$0.11 \\
JD23.28 & 28.21$\pm$0.07 & 27.11$\pm$0.02 & 27.15$\pm$0.02 & 27.32$\pm$0.03 & 28.90$\pm$0.06 & 28.74$\pm$0.10 & 28.39$\pm$0.05 & 28.46$\pm$0.09 & 28.57$\pm$0.09 \\
JD23.29 & $>$30.2        & 30.13$\pm$0.43 & 28.56$\pm$0.12 & 29.19$\pm$0.20 & 29.76$\pm$0.21 & $>$30.1        & 29.31$\pm$0.23 & 28.75$\pm$0.17 & 28.58$\pm$0.11 \\
JD23.30 & $>$30.2        & $>$30.6        & $>$30.5        & $>$30.6        & 30.03$\pm$0.11 & 29.21$\pm$0.12 & 29.05$\pm$0.08 & 28.98$\pm$0.09 & 28.92$\pm$0.08 \\
JD23.31 & 27.01$\pm$0.12 & 26.53$\pm$0.10 & 26.30$\pm$0.16 & 26.12$\pm$0.19 & 27.47$\pm$0.07 & 27.64$\pm$0.15 & 27.73$\pm$0.14 & 27.58$\pm$0.13 & 27.64$\pm$0.11 \\
JD23.32 & 29.94$\pm$0.50 & 28.93$\pm$0.19 & 29.07$\pm$0.36 & 28.28$\pm$0.12 & $>$30.7        & $>$30.1        & $>$30.6        & $>$30.1        & $>$30.3        \\
JD23.33 & 26.92$\pm$0.02 & 26.71$\pm$0.01 & 26.45$\pm$0.01 & 26.59$\pm$0.02 & 26.85$\pm$0.02 & 27.11$\pm$0.02 & 27.03$\pm$0.02 & 27.33$\pm$0.04 & 27.42$\pm$0.05 \\
JD23.34 & $>$30.2        & 30.27$\pm$0.23 & 30.07$\pm$0.20 & 29.74$\pm$0.17 & 30.22$\pm$0.18 & $>$30.1        & $>$30.6        & $>$30.1        & $>$30.3        \\
JD23.35 & 28.94$\pm$0.28 & 27.97$\pm$0.06 & 26.49$\pm$0.02 & 25.87$\pm$0.04 & 26.13$\pm$0.07 & 26.27$\pm$0.09 & 26.22$\pm$0.08 & 26.61$\pm$0.10 & 26.90$\pm$0.11 \\
JD23.36 & \nodata        & \nodata        & \nodata        & \nodata        & 27.62$\pm$0.10 & 28.23$\pm$0.18 & 28.17$\pm$0.14 & 28.67$\pm$0.22 & 28.24$\pm$0.12 \\
JD23.37 & $>$30.2        & 29.60$\pm$0.23 & 29.49$\pm$0.20 & \nodata        & 29.10$\pm$0.10 & $>$30.1        & 29.94$\pm$0.19 & 29.41$\pm$0.25 & 29.64$\pm$0.21 \\
JD23.38 & 29.48$\pm$0.26 & 29.35$\pm$0.15 & 30.28$\pm$0.32 & 29.59$\pm$0.19 & 30.50$\pm$0.23 & $>$30.1        & $>$30.6        & $>$30.1        & $>$30.3         \\ \hline
\enddata

\label{tab_JD23_photometry}

\end{deluxetable}
\end{longrotatetable}

==> tab/tab_epoch3_aperture_phot.tex <==
%\begin{longrotatetable}
\begin{deluxetable*}{ccccccccc}
\tablewidth{0pt}
\tablecaption{JD23 Epoch3-Epoch1 SN photometry}
\tablehead{
\colhead{ID} & \colhead{F090W} & \colhead{F115W} & \colhead{F150W} & \colhead{F200W} & \colhead{F277W} & \colhead{F356W} & \colhead{F410M} & \colhead{F444W} \\
\colhead{} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)}
} 
\label{tab_E3_photometry}
\startdata
JD23.2  & $>$29.4        & $>$29.9        & $>$29.8        & $>$29.8        & 29.62$\pm$0.16 & 29.54$\pm$0.18 & $>$29.1        & $>$29.2        \\
JD23.4  & $>$29.4        & $>$29.9        & 29.70$\pm$0.41 & 29.76$\pm$0.33 & 29.40$\pm$0.17 & 29.75$\pm$0.22 & $>$29.1        & $>$29.2        \\
JD23.7  & $>$29.4        & $>$29.9        & $>$29.8        & 29.46$\pm$0.39 & 28.14$\pm$0.19 & 28.68$\pm$0.24 & 28.43$\pm$0.21 & 28.66$\pm$0.28 \\
JD23.9  & $>$29.4        & $>$29.9        & $>$29.8        & 29.57$\pm$0.23 & 28.85$\pm$0.09 & 28.96$\pm$0.09 & 28.65$\pm$0.12 & $>$29.2        \\
JD23.10 & $>$29.4        & 29.69$\pm$0.30 & 27.36$\pm$0.04 & 26.59$\pm$0.03 & 26.94$\pm$0.03 & 26.89$\pm$0.03 & 27.07$\pm$0.05 & 27.17$\pm$0.05 \\
JD23.11 & $>$29.4        & $>$29.9        & 29.55$\pm$0.32 & 28.83$\pm$0.16 & 28.51$\pm$0.06 & 28.57$\pm$0.06 & 28.75$\pm$0.15 & 28.49$\pm$0.09 \\
JD23.19 & $>$29.4        & $>$29.9        & 29.16$\pm$0.18 & 28.23$\pm$0.08 & 28.38$\pm$0.06 & 28.56$\pm$0.06 & $>$29.1        & 28.60$\pm$0.09 \\
JD23.23 & 28.92$\pm$0.30 & 28.81$\pm$0.24 & 28.41$\pm$0.17 & 29.30$\pm$0.33 & $>$29.7        & $>$29.8        & $>$29.1        & $>$29.2        \\
JD23.24	& $>$29.4        & $>$29.9        & 28.19$\pm$0.17 & 27.67$\pm$0.11 & 26.72$\pm$0.12 & 27.02$\pm$0.20 & 26.91$\pm$0.23 & 27.71$\pm$0.54 \\
JD23.26 & 28.59$\pm$0.17 & 27.23$\pm$0.04 & 27.17$\pm$0.04 & 27.22$\pm$0.04 & 27.49$\pm$0.04 & 27.92$\pm$0.06 & 27.86$\pm$0.10 & 27.91$\pm$0.09 \\
\enddata



\end{deluxetable*}
%\end{longrotatetable}

==> tab/tab_epoch4_aperture_phot.tex <==
%\begin{longrotatetable}
\begin{deluxetable*}{ccccccccc}
\tablecaption{JD23 Epoch4-Epoch1 SN photometry}
\tablehead{
\colhead{ID} & \colhead{F115W} & \colhead{F150W} & \colhead{F200W} & \colhead{F277W} & \colhead{F356W} & \colhead{F444W} \\
\colhead{} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)}
} 
\label{tab_E4_photometry}
\startdata
JD23.1  & $>$28.6        & $>$28.9        & $>$29.0        & $>$28.9        & 28.93$\pm$0.22 & $>$28.4        \\
JD23.2  & $>$28.6        & $>$28.9        & $>$29.0        & $>$28.9        & 29.02$\pm$0.15 & $>$28.4        \\
JD23.4  & $>$28.6        & $>$28.9        & $>$29.0        & $>$28.9        & $>$28.9        & $>$28.4        \\
JD23.5  & $>$28.6        & $>$28.9        & $>$29.0        & $>$28.9        & $>$28.9        & $>$28.4        \\
JD23.6  & $>$28.6        & $>$28.9        & 28.40$\pm$0.18 & 28.15$\pm$0.09 & 28.15$\pm$0.09 & 28.58$\pm$0.21 \\
JD23.8  & $>$28.6        & $>$28.9        & $>$29.0        & $>$28.9        & $>$28.9        & $>$28.4        \\
JD23.9  & $>$28.6        & $>$28.9        & $>$29.0        & $>$28.9        & 29.06$\pm$0.14 & $>$28.4        \\
JD23.10 & $>$28.6        & 27.78$\pm$0.11 & 26.62$\pm$0.04 & 26.65$\pm$0.03 & 26.80$\pm$0.04 & 27.08$\pm$0.06 \\
JD23.11 & $>$28.6        & $>$28.9        & 29.09$\pm$0.33 & 28.53$\pm$0.12 & 28.39$\pm$0.08 & $>$28.4        \\
JD23.12 & $>$28.6        & $>$28.9        & $>$29.0        & $>$28.9        & $>$28.9        & $>$28.4        \\
JD23.14	& $>$28.6        & $>$28.9        & 28.47$\pm$0.24 & 28.28$\pm$0.14 & 28.54$\pm$0.20 & 28.42$\pm$0.18 \\
JD23.15 & $>$28.6        & $>$28.9        & 28.52$\pm$0.18 & 28.15$\pm$0.09 & 27.81$\pm$0.06 & 28.45$\pm$0.16 \\
JD23.17	& $>$28.6        & 28.66$\pm$0.30 & 28.43$\pm$0.23 & 28.57$\pm$0.22 & 28.47$\pm$0.14 & $>$28.4        \\
JD23.18 & $>$28.6        & $>$28.9        & 29.17$\pm$0.34 & 28.61$\pm$0.12 & 28.93$\pm$0.17 & $>$28.4        \\
JD23.19 & $>$28.6        & $>$28.9        & 28.19$\pm$0.14 & 28.29$\pm$0.08 & 28.53$\pm$0.10 & $>$28.4        \\
JD23.22	& $>$28.6        & 28.72$\pm$0.30 & 28.31$\pm$0.20 & 28.14$\pm$0.07 & 27.97$\pm$0.08 & 28.18$\pm$0.13 \\
JD23.23 & $>$28.6        & 28.72$\pm$0.41 & $>$29.0        & $>$28.9        & $>$28.9        & $>$28.4        \\
JD23.24	& $>$28.6        & 28.50$\pm$0.29 & 27.78$\pm$0.15 & 26.68$\pm$0.10 & 27.68$\pm$0.42 & 27.75$\pm$0.73 \\
JD23.26 & 27.45$\pm$0.13 & 27.36$\pm$0.08 & 27.09$\pm$0.06 & 27.48$\pm$0.05 & 28.08$\pm$0.10 & 27.95$\pm$0.12 \\
JD23.27 & $>$28.6        & $>$28.9        & $>$29.0        & $>$28.9        & 28.58$\pm$0.10 & $>$28.4        \\
JD23.30 & $>$28.6        & $>$28.9        & $>$29.0        & $>$28.9        & $>$28.9        & $>$28.4        \\
JD23.35 & 28.54$\pm$0.43 & 26.42$\pm$0.06 & 26.58$\pm$0.08 & 25.90$\pm$0.09 & 26.26$\pm$0.13 & 27.07$\pm$0.22 \\
JD23.38 & $>$28.6        & $>$28.9        & $>$29.0        & $>$28.9        & $>$28.9        & $>$28.4        \\
\enddata

\end{deluxetable*}
%\end{longrotatetable}

==> tab/tab_epoch5.2_aperture_phot.tex <==
%\begin{longrotatetable}
\begin{deluxetable*}{ccccccccc}
\tablecaption{JD23 Epoch5-Epoch1 SN photometry}
\tablehead{
\colhead{ID} & \colhead{F150W} & \colhead{F200W} & \colhead{F277W} & \colhead{F356W} & \colhead{F444W} \\
\colhead{} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)} & \colhead{(AB mag)}
} 
\label{tab_E5_photometry}
\startdata
JD23.1  & $>$28.9        & $>$29.3        & $>$28.9        & $>$28.9        & $>$28.4        \\
JD23.2  & $>$28.9        & $>$29.3        & $>$28.9        & 28.96$\pm$0.17 & $>$28.4        \\
JD23.4  & $>$28.9        & $>$29.3        & 28.90$\pm$0.15 & $>$28.9        & $>$28.4        \\
JD23.6  & $>$28.9        & 29.09$\pm$0.23 & 28.32$\pm$0.11 & 28.11$\pm$0.07 & $>$28.4        \\
JD23.7  & 28.69$\pm$0.26 & 27.99$\pm$0.14 & 27.71$\pm$0.16 & 28.74$\pm$0.32 & 28.18$\pm$0.18 \\
JD23.9  & $>$28.9        & $>$29.3        & 28.81$\pm$0.11 & $>$28.9        & $>$28.4        \\
JD23.10 & 28.34$\pm$0.17 & 27.04$\pm$0.04 & 26.93$\pm$0.03 & 26.79$\pm$0.03 & 27.07$\pm$0.07 \\
JD23.11 & $>$28.9        & 29.34$\pm$0.30 & 28.64$\pm$0.11 & 28.50$\pm$0.10 & $>$28.4        \\
JD23.12 & $>$28.9        & 29.31$\pm$0.29 & 29.31$\pm$0.20 & $>$28.9        & $>$28.4        \\
JD23.14	& $>$28.9        & 28.91$\pm$0.33 & 28.67$\pm$0.21 & 28.60$\pm$0.20 & 28.59$\pm$0.30 \\
JD23.15 & $>$28.9        & 28.52$\pm$0.16 & 28.24$\pm$0.09 & 28.04$\pm$0.06 & 28.57$\pm$0.17 \\
JD23.17	& 28.83$\pm$0.32 & 29.06$\pm$0.29 & $>$28.9        & $>$28.9        & $>$28.4        \\
JD23.18 & $>$28.9        & 28.82$\pm$0.17 & 28.82$\pm$0.16 & 28.79$\pm$0.12 & $>$28.4        \\
JD23.19 & $>$28.9        & 28.49$\pm$0.12 & 28.71$\pm$0.12 & 28.87$\pm$0.14 & $>$28.4        \\
JD23.20 & $>$28.9        & $>$29.3        & $>$28.9        & $>$28.9        & $>$28.4        \\
JD23.22 & $>$28.9        & 28.44$\pm$0.13 & \nodata        & \nodata        & \nodata        \\
JD23.23 & $>$28.9        & 29.14$\pm$0.28 & $>$28.9        & $>$28.9        & $>$28.4        \\
JD23.24 & $>$28.9        & 28.05$\pm$0.14 & 27.07$\pm$0.10 & 28.51$\pm$0.69 & 27.52$\pm$0.36 \\
JD23.26 & 27.41$\pm$0.10 & 27.14$\pm$0.05 & 27.39$\pm$0.06 & 27.84$\pm$0.11 & 28.45$\pm$0.25 \\
JD23.29 & 28.20$\pm$0.18 & $>$29.3        & $>$28.9        & $>$28.9        & $>$28.4        \\
JD23.32 & 27.81$\pm$0.19 & 28.25$\pm$0.36 & 27.51$\pm$0.37 & $>$28.9        & $>$28.4        \\
JD23.33 & 26.37$\pm$0.03 & 26.37$\pm$0.03 & 26.88$\pm$0.03 & 26.93$\pm$0.04 & 27.27$\pm$0.07 \\
JD23.35 & 26.89$\pm$0.12 & 27.06$\pm$0.09 & 26.53$\pm$0.14 & 27.68$\pm$0.43 & 28.08$\pm$0.37 \\
JD23.38 & $>$28.9        & $>$29.3        & $>$28.9        & $>$28.9        & $>$28.4        \\
\enddata

\end{deluxetable*}
%\end{longrotatetable}

==> tab/tab_local_oversubtraction_corrections.tex <==
\begin{deluxetable*}{ccccccccc}
\tablecaption{0.1$^{\prime\prime}$-0.2$^{\prime\prime}$ Radius Annulus Local Background Over-Subtraction Corrections}
\tablehead{
\colhead{F090W} & \colhead{F115W} & \colhead{F150W} & \colhead{F200W} & \colhead{F277W} & \colhead{F335M} &  \colhead{F356W} & \colhead{F410M} & \colhead{F444W} 
} 
\label{tab_local_oversub}
\startdata
1.024 & 1.025 & 1.025 & 1.028 & 1.087 & 1.095 & 1.097 & 1.093 & 1.126 \\
\enddata
\end{deluxetable*}
